Slippage-robust Gaze Tracking for Near-eye Display

In recent years, head-mounted near-eye display devices have become the key hardware foundation for virtual reality and augmented reality. Thus head-mounted gaze tracking technology has received attention as an essential part of human-computer interaction. However, unavoidable slippage of head-mounted devices (HMD) often results higher gaze tracking errors and hinders the practical usage of HMD. To tackle this problem, we propose a slippage-robust gaze tracking for near-eye display method based on the aspheric eyeball model and accurately compute the eyeball optical axis and rotation center. We tested several methods on datasets with slippage and the experimental results show that the proposed method significantly outperforms the previous method (almost double the suboptimal method).

==> Section/abstract.tex <==
Eye tracking technique has been adopted in near-eye display systems for various purposes, including virtual reality rendering optimization, optical see-through display calibration and human computer interaction. However, most existing studies choose to combine commercial head-mounted eye trackers and few works focus on near-eye displayed eye tracking. Here, we introduce a slippage-robust eye tracking system for near-eye display. On the basis of a proposed eye model, a hardware implementation is presented with eyeball optical axis and eyeball rotation center detection method. By modeling the relation between eyeball features and gaze point in near-eye display, a slippage-robust gaze estimation method is proposed. Calibration and validation experiments have been conducted on 9 subjects. Results show that the proposed method acquires a stable and accurate eyeball optical axis and rotation center detection and maintains high gaze estimation accuracy when head-mounted device slippage occurs. 

==> Section/introduction.tex <==
With the popularity of the metaverse concept, human-centric headsets such as augmented, virtual and mixed reality are showing rapid development. Head-mounted devices project virtual scenes onto the human eye, thus creating an immersive environment. A natural movement in head-mounted devices is the eye gaze movement, and our behavior and intention can be recognized from the way we move our eyes, thus head-mounted near-eye vision tracking technology shows great potential in the field of human-computer interaction.


With the popularization of the concept of metaverse, a promising future of augmented, virtual and mixed reality (AR, VR and MR) predictable. Due to the advantages including low cost, portable device and highly immersive experience, head-mounted display (HMD) devices turned out to be the best-accepted solution of current AR and VR. The near-eye display system in HMD projects virtual scenes to human eyes to build up an immersive environment. However, except visual scene, the rest of user's body and senses remain in the real world, which means all motions and feelings will be different from those in usual practice. One natural motion in HMD is eye gaze movement. Thanks to head-mounted eye tracking techniques, a better user experience in AR and VR is possible to be obtained by leveraging eyeball and gaze information. Eye tracking techniques utilized in near-eye display can be classified into eyeball tracking and gaze estimation. 

Eyeball features indicate user's eye position and eye pose. According to near-eye display principle, eyeball must lie on a correct position to achieve the ideal visual appearance and visual angle. False eye position might cause image distortion in VR~\cite{jones2015correction} and object misalignment in MR. Detection of eye position and online rendering correction will significantly improve near-eye display user experience. An eye pose estimation method~\cite{nitschke2011image} was adopted in interaction-free AR calibration method~\cite{itoh2014interaction} for eye position acquisition while predefined eyeball parameters introduce deviation among people. Estimating eyeball rotation center with eye poses was discussed in gaze tracking~\cite{swirski2013fully} as well, but the result was highly dependent on pupil contour tracking. A robust eyeball position estimation for various persons still remains a problem in head-mounted systems. 

Based on knowledge of human gaze mode in real environment, gaze-based improvements in graphic rendering and displaying~\cite{patney2016towards,konrad2020gaze,krajancich2020optimizing} have been studied. Furthermore, human gaze directly indicates human perceptions and attention, which is suitable for human-computer interaction. Gaze cues have already been adopted in interactions between human and smart
systems~\cite{zheng2018rapid,majaranta2019eye,saran2018human} and similar interaction studies have been conducted on AR/VR devices with gaze tracking implementation. Results show that gaze-base interaction promises higher interaction quality, higher interaction speed and more user-friendly experience~\cite{blattgerste2018advantages}. Unfortunately, in common AR/VR application scenarios, body motions and head motions constantly exist during
practical use, which leads to an unavoidable HMD slippage and slight slippage often results in a significant increase in gaze estimation error of head-mounted devices~\cite{li2020optical,clay2019eye}. Most commercial eye trackers also suffer from the accuracy degradation caused by slippage~\cite{niehorster2020impact}. Methods to maintain gaze accuracy after slippage have been investigated~\cite{santini2019get} and results show the robustness to headset slippage in head-mounted gaze tracking. However, the overall gaze estimation accuracy of slippage-robust methods are lower than most state-of-the-art methods and only qualified for limited uses. Another gap between present works and the need is that most gaze tracking studies about slippage were conducted in real world space. When viewing near-eye display, binocular collaboration mechanism might be different from viewing real world objects and might change the gaze tracking model. 

In this work, we proposed a slippage-robust eye tracking system for near-eye displays which is suitable for practical head-mounted AR/VR. A head-mounted hardware setup is proposed and robust three dimensional eye features, including eyeball axes and eye positions, are extracted from collected eye images. The gaze model for near-eye display is proposed to estimate gaze point in rendered scene with the obtained eye features. Since two eyes are gazing at two separate displays and focusing on a same target, both eyes gazing direction need to be estimated separately. The binocular gaze results are acquired from both eyes monocular results. Experiments were conducted on multiple subjects by asking them to remount and rotate device repeatedly to simulate slippage in actual use. Results show that our proposed method achieved the state-of-the-art gaze estimation accuracy in head-mounted near-eye display and remained accurate when slippage occurred. 

==> Section/related_works.tex <==
To illustrate the importance and challenge of slippage-robust eye tracking for near-eye display, a brief survey of previous works on near-eye display eye tracking and slippage-robust gaze estimation is given.

\subsection{Eye Tracking in Near-eye Display}

Near-eye display provide an immersive visual experience by directly projecting rendered scene to human eyes. Precisely tracking eyeball position and gaze direction will extract useful information for near-eye display imaging to elevate user experience. 

Originally, eyeball position estimation was an crucial topic in gaze tracking since eyeball optical axis and line of sight contain several key points of eyeball (e.g. pupil center, cornea center, rotation center). Based on a simple eyeball model with spherical cornea~\cite{lee2009robust}, corneal reflections produced by infrared LEDs assisted to construct normal vectors of cornea surface and calculate cornea center. The scheme of corneal imaging with near-eye display utilized a more complex pattern~\cite{plopski2015corneal} to achieve higher accuracy. However, due to a relatively large error introduced by model approximation, eyeball locating methods considered pupil as a more accurate feature. Pupil reprojection built a three-dimensional surface and estimated eyeball optical axis~\cite{swirski2013fully}. Multiple optical axes gave a eyeball rotation center estimation according to the eye rotation rule. Similar method was adopted in optical see-through display calibration~\cite{itoh2014interaction}. 

On the other hand, gaze estimation is a more widely-known topic. Gaze direction points at the information being received. A natural gaze phenomenon is that the central of field of view obtains a higher resolution than the outer parts because the view around fixation point is imaged on foveal~\cite{hunter1999automated}, the most sensitive region on retina. Foveated rendering in near-eye display~\cite{tan2018foveated,patney2016towards,gao2021foveated} aims to imitate this physiological phenomenon to lower computation cost of graphic rendering and offer a better user experience. Higher accuracy of gaze tracking is likely to provide further promotion in foveated imaging and rendering~\cite{matthews2020rendering}. Gaze-contingent near-eye display rendering also performed better in parallax construction and depth perception optimization~\cite{krajancich2020optimizing,konrad2020gaze}. Binocular gaze information was proved to be useful for stereoscopic perception~\cite{liu2021perceptual}. Besides, gaze also implies user intention and thus, gaze estimation show great potential in human computer interaction in near-eye display~\cite{rajanna2018gaze,piumsomboon2017exploring} in the near future. 

Research results exhibited a strong eye tracking demand in near-eye display scenarios. 

\subsection{Slippage-robust Gaze Estimation}

Head-mounted gaze estimation is the basis of gaze-contingent near-eye display realization. A defect of most existing head-mounted gaze tracking methods is the lack of slippage robustness. During a common use, a relative slight movement between head-mounted device and eyes is unavoidable. Keeping high gaze estimation accuracy with slippage taken in consideration should be realized in practical head-mounted systems. 

Model-based gaze tracking methods~\cite{lukander2013omg} are often considered robust to device slippage but complicated system calibration and relatively low accuracy made these methods less popular. State-of-the-art feature-based gaze estimation method proposed by PupilLab~\cite{kassner2014pupil} achieved a mean angular error lower than $0.6^{\circ}$. Combination of PupilLab eye tracker and VR systems have been studied~\cite{clay2019eye,piumsomboon2017exploring}. However, the method purely relied on 2D pupil feature and was highly sensitive to slippage. The commonly accepted slippage-robust gaze tracking method Grip~\cite{santini2019get} used model-based feature (optical axis) and feature-based gaze mapping model. An acceptable gaze accuracy with slippage robustness was shown. End-to-end learning-based gaze estimation method~\cite{tonsen2017invisibleeye} was proved to be robust and accurate when headset slippage occurred, but model training was data consuming and required users to collect a large amount of calibration data. 

Recently, slippage in head-mounted gaze tracking has become a critical research problem and increasing works have been aware of the importance of slippage robustness. Still, few works discussed slippage-robust near-eye display gaze tracking. 
